Towards Reproducible Network Traffic Analysis

Analysis techniques are critical for gaining insight into network traffic given both the higher proportion of encrypted traffic and increasing data rates. Unfortunately, the domain of network traffic analysis suffers from a lack of standardization, leading to incomparable results and barriers to reproducibility. Unlike other disciplines, no standard dataset format exists, forcing researchers and practitioners to create bespoke analysis pipelines for each individual task. Without standardization researchers cannot compare "apples-to-apples", preventing us from knowing with certainty if a new technique represents a methodological advancement or if it simply benefits from a different interpretation of a given dataset. In this work, we examine irreproducibility that arises from the lack of standardization in network traffic analysis. First, we study the literature, highlighting evidence of irreproducible research based on different interpretations of popular public datasets. Next, we investigate the underlying issues that have lead to the status quo and prevent reproducible research. Third, we outline the standardization requirements that any solution aiming to fix reproducibility issues must address. We then introduce pcapML, an open source system which increases reproducibility of network traffic analysis research by enabling metadata information to be directly encoded into raw traffic captures in a generic manner. Finally, we use the standardization pcapML provides to create the pcapML benchmarks, an open source leaderboard website and repository built to track the progress of network traffic analysis methods.

==> figures/tables/future/terms.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
    \centering
\begin{tabular}{@{}cl@{}}
\toprule
\textbf{Term} & \multicolumn{1}{c}{\textbf{Defined As}}                                                              \\ \midrule
Flow          & 5-tuple (source IP, destination IP, source port, destination port), unidrectional                                       \\
Application   & Single flow, determined by the flow with the highest number of packets while running the applicaiton \\ \bottomrule
\end{tabular}
\caption{Clear terminology will help ground readers and contextualize methods.}
\label{tab:clearterms}
\end{table*}


==> sections/future.tex <==
\section{Future Directions}

Although we believe \sys{} provides significant improvements
to the reproducibility of network traffic analysis research, there 
are multiple avenues for future work. One natural direction forward is to increase
the scale at which \sys{} can capture and tag live network traffic. Although
\sys{} can capture and encode at rates viable for many experiments, attaching
metadata on any high-speed link, such as a campus network, is currently not 
feasible. One possible way to increase the scalability of \sys{} is to leverage
kernel-level networking capabilities, such as eBPF~\cite{ebpf}.

Another area for future work involves more complete benchmarking of traffic
analysis tasks. Many of these extensions involve implementing practices 
already used in other domains, such as image recognition. ``Model zoos'', in 
which machine learning models can be loaded and tested in a single line of 
code, are an extension to the \sys{} benchmarks that would further improve 
reproducibility~\cite{croce2020robustbench}.

